SN2020qlb: A hydrogen-poor superluminous supernova with well-characterized light curve undulations

SN\,2020qlb (ZTF20abobpcb) is a hydrogen-poor superluminous supernova (SLSN-I) that is among the most luminous (maximum M$_{g} = -22.25$ mag) and that has one of the longest rise times (77 days from explosion to maximum). We estimate the total radiated energy to be $>2.1\times10^{51}$ erg. SN\,2020qlb has a well-sampled light curve that exhibits clear near and post peak undulations, a phenomenon seen in other SLSNe, whose physical origin is still unknown. We discuss the potential power source of this immense explosion as well as the mechanisms behind its observed light curve undulations. We analyze photospheric spectra and compare them to other SLSNe-I. We constructed the bolometric light curve using photometry from a large data set of observations from the Zwicky Transient Facility (ZTF), Liverpool Telescope (LT), and Neil Gehrels Swift Observatory and compare it with radioactive, circumstellar interaction and magnetar models. Model residuals and light curve polynomial fit residuals are analyzed to estimate the undulation timescale and amplitude. We also determine host galaxy properties based on imaging and spectroscopy data, including a detection of the [O III]$\lambda$4363, auroral line, allowing for a direct metallicity measurement. We rule out the Arnett $^{56}$Ni decay model for SN\,2020qlb's light curve due to unphysical parameter results. Our most favored power source is the magnetic dipole spin-down energy deposition of a magnetar. Two to three near peak oscillations, intriguingly similar to those of SN\,2015bn, were found in the magnetar model residuals with a timescale of $32\pm6$ days and an amplitude of 6$\%$ of peak luminosity. We rule out centrally located undulation sources due to timescale considerations; and we favor the result of ejecta interactions with circumstellar material (CSM) density fluctuations as the source of the undulations.

==> tab_hostcat.tex <==
\begin{table}
\caption{Host galaxy photometry. Magnitudes are not corrected for reddening.}\label{tab:hostphot}
\tiny
\begin{tabular}{cccc}
\toprule
Instrument/Filter & Brightness & Instrument/Filter & Brightness\\
& (mag) & & (mag) \\
\midrule
%GALEX/FUV     &$22.40 \pm 0.70$ & PS1/$g$ &$22.01 \pm 0.24$\\
%GALEX/NUV     &$22.42 \pm 0.59$ & PS1/$r$ &$22.20 \pm 0.52$\\
%UVOT/$w2$     &$22.87 \pm 0.33$ & PS1/$i$ &$22.12 \pm 0.20$\\
%UVOT/$m2$     &$22.79 \pm 0.28$ & LS/$g$  &$22.13 \pm 0.10$\\
%UVOT/$w1$     &$22.34 \pm 0.51$ & LS/$r$  &$21.62 \pm 0.07$\\
%SDSS/$g$      &$22.50 \pm 0.19$ & LS/$z$  &$22.17 \pm 0.30$\\
%SDSS/$r$      &$21.52 \pm 0.16$\\
HST/$F336W$   &$23.07 \pm 0.04$ & PS1/$i$ &$22.12 \pm 0.20$\\
SDSS/$g$      &$22.50 \pm 0.19$ & LS/$g$  &$22.13 \pm 0.10$\\ 
SDSS/$r$      &$21.52 \pm 0.16$ & LS/$r$  &$21.62 \pm 0.07$\\ 
PS1/$g$       &$22.01 \pm 0.24$ & LS/$z$  &$22.17 \pm 0.30$\\ 
PS1/$r$       &$22.20 \pm 0.52$ & \\ 
\bottomrule
\end{tabular}
\end{table}

